PROMPTEVALS: A Dataset of Assertions and Guardrails for Custom Production Large Language Model Pipelines

Large language models (LLMs) are increasingly deployed in specialized production data processing pipelines across diverse domains -- such as finance, marketing, and e-commerce. However, when running them in production across many inputs, they often fail to follow instructions or meet developer expectations. To improve reliability in these applications, creating assertions or guardrails for LLM outputs to run alongside the pipelines is essential. Yet, determining the right set of assertions that capture developer requirements for a task is challenging. In this paper, we introduce PROMPTEVALS, a dataset of 2087 LLM pipeline prompts with 12623 corresponding assertion criteria, sourced from developers using our open-source LLM pipeline tools. This dataset is 5x larger than previous collections. Using a hold-out test split of PROMPTEVALS as a benchmark, we evaluated closed- and open-source models in generating relevant assertions. Notably, our fine-tuned Mistral and Llama 3 models outperform GPT-4o by 20.93% on average, offering both reduced latency and improved performance. We believe our dataset can spur further research in LLM reliability, alignment, and prompt engineering.

==> figures/promptexamples.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}[node distance=1cm and 0.5cm, auto]

% Define styles
\tikzset{prompt/.style={rectangle, draw, fill=blue!5, text width=11em, align=center, rounded corners, minimum height=16em, font=\small}}

% Place nodes
\node [prompt] (programming) {{\bf Programming Prompt:}\\
You are an AI Assistant expert at reviewing pull requests. Review the pull request in Github diff format...Take into account that you don’t have access to the full code but only the code diff...Make it personal and always show gratitude to the author using ``@''...Include code snippets if necessary...};

\node [prompt, right=of programming] (medical) {{\bf Medical Prompt:}\\
You are a medical scribe for asthetic. Hear the conversation between doctor and parient. extract information using {schema}: {tools} Use following definition to extract the information: reason for visit - why patient has visited the facility. Diagnosis - what care provider has diagnosed. Treatment - description of treatment with periods...Begin! Question:...};

\node [prompt, right=of medical] (legal) {{\bf Legal Prompt:}\\
You are a world class researcher, do detailed research on legal and regulatory considerations in the {sourcing\_material} industry...Never start your answers with "As an AI language model" when responding to questions...Your answers should be on point, succinct and useful. Each response should be written with maximum usefulness in mind rather than being polite...};

% Draw edges
% \draw[-Latex] (programming.east) -- (medical.west);
% \draw[-Latex] (medical.east) -- (legal.west);

\end{tikzpicture}
    \caption{Examples of prompts for custom tasks from 3 different domains. Each prompt is intended to be used as part of a bigger software product. \shreya{TODO: fix alignment} \agp{I think using this space to list an exampple custom prompt and ``good'' assertion criteria would be better.}}
    \label{fig:prompt-examples}
\end{figure}
